Empirical Analysis of Limits for Memory Distance in Recurrent Neural Networks

Common to all different kinds of recurrent neural networks (RNNs) is the intention to model relations between data points through time. When there is no immediate relationship between subsequent data points (like when the data points are generated at random, e.g.), we show that RNNs are still able to remember a few data points back into the sequence by memorizing them by heart using standard backpropagation. However, we also show that for classical RNNs, LSTM and GRU networks the distance of data points between recurrent calls that can be reproduced this way is highly limited (compared to even a loose connection between data points) and subject to various constraints imposed by the type and size of the RNN in question. This implies the existence of a hard limit (way below the information-theoretic one) for the distance between related data points within which RNNs are still able to recognize said relation.

==> authors_blind.tex <==
\author{\authorname{
Double Blind \sup{1},
Double Blind \sup{1},
Double Blind\sup{1},
Double Blind \sup{1} and 
Double Blind \sup{1}}
\affiliation{\sup{1}Institute for Informatics, Street, City, Country}
\email{blind@mail.local}
}

==> backstack.tex <==
\subsection{Fixed-Length Random Memorization}

We now briefly discuss the scenario of Definition~\ref{def:mem-fixed}: In this case, we fix the length of the random sequence $q = 10$, meaning that in theory it is possible to count the positions from the start and thus know exactly when the currently processed piece of the input data stream needs to be memorized, sparing the effort of memorizing as many of them as possible until the end. We thus consider this task strictly easier and our experimental results shown in Figure~\ref{fig:RNN-static} support this. However, the strategy of ``counting from the start'' seems to be subject to some memory limitations as well. Thus, while every instance that is easily learned in the case of variable-length sequences is also learnable in this scenario, further learnable instances appear from the right of the plot, i.e., $p = 10$ for the 1-layer 2-cells network and $p \geq 8$ for the 2-layers 2-cells-each network. This shows that the RNN is not exactly able to count through the sequence but again memorizes pieces from the start, within a very similar limit as from the end of the sequence. As LSTMs show a very similar behavior, we omit the respective plots for brevity.

\begin{figure*}[t]
	\centering
	\includegraphics[width=.7\textwidth]{results/rnn_static}
	\caption{Mean absolute loss for various configurations of \textbf{RNNs} % with $l \in \{1,2,3\} $ layers with $c \in [1;10]$ cells each when asked to reproduce the $p$th-from-last position (for $p \in [1;10]$) 
	trained on a random sequences of fixed length $q = 10$.}
	\label{fig:RNN-static}
\end{figure*}

\subsection{Correlated Memorization Task}

Much closer to the original intention behind using RNNs is the task of correlated memorization as given in Definition~\ref{def:cor-mem}. Here, we build a random sequence in such a way that the elements of the sequence are highly correlated, allowing us to deduce even the initial element at $p = q$ to some extent from the last given element at $p = 1$. Again, we conducted the same suite of experiments for different configurations of RNNs, as shown in Figure~\ref{fig:RNN_CORR}. Matching our expectation, this setup becomes much easier for the RNNs and they can reproduce the entire sequence almost perfectly even using just $c = 3$ cells on $l = 1$ layers. Interestingly, despite the correlation decreasing towards the beginning of the sequence (cf. Section~\ref{sec:methodology}), the RNNs with $c = 2$ cells and $l \in \{1,2,3\}$ layers still show a tendency to memorize the beginning of the sequence ($p = 10$) first. 
Furthermore, we show the same experiments for LSTMs in Figure~\ref{fig:LSTM_CORR}. Here, it clearly shows that LSTMs outperform RNNs, almost perfectly reproducing any sequence except those in the bottom rows. Despite their additional weights and free parameters to train, LSTMs apparently make better use of the correlation present in the data sequence to learn better approximations in the same amount of time.

\begin{figure*}[tb]
	\begin{minipage}[t]{.48\textwidth}
		\includegraphics[width=.9\textwidth]{results/rnn_corr}
		\caption{Mean absolute loss for various configurations of \textbf{RNNs} with $l \in \{1,2,3\}$ layers with $c \in [1;10]$ cells each when asked to reproduce the $p$th-from-last position (for $p \in [1;10]$) of a semi-random correlated sequence of random length $q \in [10;15]$. Every data point is averaged over $10$ runs.}
		\label{fig:RNN_CORR}
	\end{minipage}%
	\hfill
	\begin{minipage}[t]{.48\textwidth}
		\includegraphics[width=.9\textwidth]{results/lstm_corr}
		\caption{Mean absolute loss for various configurations of \textbf{LSTMs} with $l \in \{1,2,3\}$ layers with $c \in [1;10]$ cells each when asked to reproduce the $p$th-from-last position (for $p \in [1;10]$) of a semi-random correlated sequence of random length $q \in [10;15]$. Every data point is averaged over $10$ runs.}
		\label{fig:LSTM_CORR}
	\end{minipage}%
\end{figure*}

\iffalse
These task definitions are in stark contrast to common applications of RNNs where one explicitly expects some connections or correlations between the pieces of the input sequence and thus uses RNNs to approximate a model of said connections. We further define a task which explicitly models such correlations:

\begin{mydef}[Correlated Memorization Task]
\label{def:cor-mem}
	Let $q=10$.
	Let $\mathbf{y} = \langle{y_i}\rangle_{1 \leq i \leq q, i \in \mathbb{N}}$ be a sequence of random numbers $y_i$ each uniformly sampled from $[0;1] \subseteq \mathbb{R}$. Let $\mathbf{x} = \langle{x_i}\rangle_{1 \leq i \leq q, i \in \mathbb{N}}$ be a sequence so that $x_1 = y_1$ and $x_i = \alpha_i \cdot x_{i-1} + (1-\alpha_i) \cdot y_i$ for $2 \leq i \leq q$ and a correlation parameter $\alpha_i = \frac{i}{q}$. For all else, refer to Definition~\ref{def:mem}.
\end{mydef}

Intuitively, the correlated memorization task defines a sequence $\mathbf{x}$ so that each $x_i$ depends on the previous piece $x_{i-1}$ to $\alpha_i$ extent. We choose the setting $\alpha_i = \frac{i}{q}$ so that the first element $x_1$ of the sequence $\mathbf{x}$ still has a correlation with the last element $x_q$ as the impact of the random elements $\mathbf{y}$ diminishes throughout the sequence.

Thus, the RNN can reproduce values from past pieces much more accurately using information from more current pieces and should thus able to memorize more pieces into the past.
This formulation is much closer to the originally intended application of RNNs.

\fi

\iffalse
\subsection{Correlated Memorization Task}

Much closer to the original intention behind using RNNs is the task of correlated memorization as given in Definition~\ref{def:cor-mem}. Here, we build a random sequence in such a way that the elements of the sequence are highly correlated, allowing us to deduce even the initial element at $p = q$ to some extent from the last given element at $p = 1$. Again, we conducted the same suite of experiments for different configurations of RNNs, as shown in Figure~\ref{fig:RNN_CORR}. Matching our expectation, this setup becomes much easier for the RNNs and they can reproduce the entire sequence almost perfectly even using just $c = 3$ cells on $l = 1$ layers. Interestingly, despite the correlation decreasing towards the beginning of the sequence (cf. Section~\ref{sec:methodology}), the RNNs with $c = 2$ cells and $l \in \{1,2,3\}$ layers still show a tendency to memorize the beginning of the sequence ($p = 10$) first.

Furthermore, we show the same experiments for LSTMs in Figure~\ref{fig:LSTM_CORR}. Here, it clearly shows that LSTMs outperform RNNs, almost perfectly reproducing any sequence except those in the bottom rows. Despite their additional weights and free parameters to train, LSTMs apparently make better use of the correlation present in the data sequence to learn better approximations in the same amount of time.

\begin{figure*}[tb]
	\begin{minipage}[t]{.48\textwidth}
		\includegraphics[width=.9\textwidth]{results/rnn_corr}
		\caption{Mean absolute loss for various configurations of \textbf{RNNs} with $l \in \{1,2,3\}$ layers with $c \in [1;10]$ cells each when asked to reproduce the $p$th-from-last position (for $p \in [1;10]$) of a semi-random correlated sequence of random length $q \in [10;15]$. Every data point is averaged over $10$ runs.}
		\label{fig:RNN_CORR}
	\end{minipage}%
	\hfill
	\begin{minipage}[t]{.48\textwidth}
		\includegraphics[width=.9\textwidth]{results/lstm_corr}
		\caption{Mean absolute loss for various configurations of \textbf{LSTMs} with $l \in \{1,2,3\}$ layers with $c \in [1;10]$ cells each when asked to reproduce the $p$th-from-last position (for $p \in [1;10]$) of a semi-random correlated sequence of random length $q \in [10;15]$. Every data point is averaged over $10$ runs.}
		\label{fig:LSTM_CORR}
	\end{minipage}%
\end{figure*}

\fi

%
%Experiments	
%\begin{itemize}
%	\item Dynmische Sequenzlängen stellen eine Herausforderung für das netzwerk da, da die Zellen so nicht ab wann Sie sich etwas merken sollen.
%	\item Random Sequence generation with various random length between $[10,15]$\\
%	Random Sequence Numbers Between $[0,1]$, Normal NORMAL?????? \hl{not normal, always EQUAL} Distributions for all random calls
%	\item Random Sequence generation with fixed length between $10$?
%		Wir zeigen nur einmal weil einfache Problemstellung, wird besser gelöst, Einfluss der gleiche.
%	\item Correlated Semi-Random Sequence generation with variable length between $[10,15]$
%		Wir zeigen GRU nicht nochmal weil er LSTM ähnlich ist
%	\item Alle Runs liefen 500 Epochen, wobei jede Epoche 1000 mini-batches enthielt.\\
%		leider mussten wir die Größe der Minibatches auf 1 reduzieren, da wir dynamische aktivierungen vorgenommen hatten.
%	\item The formula for our correlated dataset goes: \\
%	We first create a random vector with shape(n, sequence length, 1), then apply the following formula
%	$$ y_i =  (1-\frac{i}{seq_len}) * x_i + \frac{i}{seq_len} * y_{i-1} \mathit{where~ i=sequence_position}$$
%		
%\end{itemize}
%
%Parameters 
%\begin{itemize}
%	
%	\item Random Equal Distribution \{0,1\} for features in the sequence
%	\item Random Equal Distribution \{0,n=5\} for dynamic sequence length (n=6 due to python stuff...)
%	
%	\item Dynamic activated RNN Cells
%	\item Loss function = Mean Squared Error
%	\item Various Parameter Configurations:
%	\begin{itemize}
%		\item Cells: \{1, 10\}
%		\item Layers: \{0, 3\}
%		\item Seeds: \{0, 10\}
%		\item Cell Types: \{RNN, LSTM, GRU\}
%	\end{itemize}
%
%	\begin{figure}
%		\includegraphics*[width=\columnwidth]{fig/architecture}
%		\label{fig:architecture}
%		\caption{Our NN-Model Architecture for n\_layers=1; n\_cells=2}
%	\end{figure}
%
%\end{itemize}

%\todo{Check $\alpha$, definition given in notes looks backwards to me right now. Why didn't we use $\alpha = .5$ again?} 
%\todo[color=blue]{This decision was made due to the variable sequence length and the Random Number Generation. 
%	With  $\alpha = .5$, the sequence would still be pretty random. 
%	But with $\alpha = i/seqLen$, we lowered te influence of every new value a result that gets more stable with every step. 
%	Check excel sheet alpha.xlsx} 


%All values are retrieved by running 10 parallel configurations, with the ever same seeds (${0, 9}$).
%Total Loss is then the Mean ( Over All Mins ( over all Total Loss Values) )
%At 0.25 Total Loss, the model is randomly guessing (since 0.5 is the outcome in most of the times).
%\begin{todolist}
%	\item RNN: \\
%	\begin{itemize}
%		\item Seems like a linear correlation between cell size and index position (training target distance)
%		\item This is True along Models with 1, 2 \& 3 layers
%		\item With more layers, the Models need less cells to get accuracies better than 0.04\% total loss
%		\item RNN was not able to learn temporal relations that were more then seven time steps away from the network output at parameter settings 8Cells, 1Layer. 
%		With increasing network complexity and cell size, RNN were able to master all tasks with 4 to 6 cells at 3 and 2 layers. 
%		We therefore assume a more sophisticated concept of distance while introducing more cells and layers.... \hl{umformulieren, zusammenhang zwischen distance und cellen bzw layern herstellen.}
%		We furthermore assume a mostly linear correlation between recurrent cells and the groups memory horizon. 
%		While layers of such introduce a .. \hl{ja was?}, ... \hl{koennen wir so etwas ueberhaupt sagen?}, ... \hl{mit den wenigen daten....?}
%	\end{itemize}
%	\item LSTM:
%		\begin{itemize}
%		\item LSTM are assumed to have the capability to outperform simple RNN cells by far. 
%		\item Our Experiments however showed, that at the given learning time at around 500 epochs of training, LSTM cells were able to learn a memory horizon of 6 time steps at about 6 cells having a single layer. 
%		\item While increasing the layer count, the network refused to learn further positional meaning, this turned out in the opposite as expected. 
%		\item We assume that an increase in recurrent LSTM Layers is a so heavy lifting for the optimizer, so that the sum of weights, that are at the factor 4 of traditional RNN Cells are not able to train to converge in given time.
%		\item We don't think that the made observations are a problem introduced by the truncated BPTT usually used to compute the gradients for weight adjustment in LSTM cells \cite{williams1990efficient,hochreiter1997long}.
%		\end{itemize}
%	\item GRU: 
%		\begin{itemize}
%			\item In Theory, GRU cells are in direct comparision to LSTM cells (the bigger brother (\hl{no scientific wording redo})) GRU Cells posses less weighted gates and are therefore able to learn relevant temporal correlations given shorter training times.  
%			\item Our experiments validate this assumption. 
%			\item While supporting our experimental setup with more layers of Gated Recurrent Units, this cells were able to learn further temporal connections (up to eight time steps at 8 cells).		 
%		\end{itemize}
%\end{todolist}
%
%
%
%We found that RNN \% LSTM cells converged faster and with a higher absolute loss in experiments when correlated data structures were omitted.
%\(  \)
%\begin{itemize}
%	\item RNN: 
%	\item LSTM:
%\end{itemize}



